Hybrid Fusion for 802.11ax Wi-Fi-based Passive Radars Exploiting Beamforming Feedbacks

Passive Wi-Fi-based radars (PWRs) are devices that enable the localization of targets using Wi-Fi signals of opportunity transmitted by an access point. Unlike active radars that optimize their transmitted waveform for localization, PWRs align with the 802.11 amendments. Specifically, during the channel sounding session preceding a multi-user multiple-input multiple-output downlink transmission, an access point isotropically transmits a null data packet (NDP) with a known preamble. From these known symbols, client user equipments derive their channel state information and transmit an unencrypted beamforming feedback (BFF) back to the access point. The BFF comprises the right singular matrix of the channel and the corresponding stream gain for each subcarrier, which allows the computation of a beamforming matrix at the access point. In a classical PWR processing, only the preamble symbols from the NDP are exploited during the channel sounding session. In this study, we investigate multiple target localization by a PWR exploiting hybrid information sources. On one hand, the joint angle-of-departure and angle-of-arrival evaluated from the NDP. On another hand, the line-of-sight angle-of-departures inferred from the BFFs. The processing steps at the PWR are defined and an optimal hybrid fusion rule is derived in the maximum likelihood framework. Monte-Carlo simulations assess the enhanced accuracy of the proposed combination method compared to classical PWR processing based solely on the NDP, and compare the localisation performance between client and non-client targets.

==> Text/Simulation_Results_-_Copy.tex <==
\section{Simulation Results} \label{sec:sim_res}

\begin{figure*}[!t]
\centering
\subfloat[RMSE]{\includegraphics[trim=3.4cm 9.5cm 4.3cm 9.91cm,width = 0.42\textwidth]{Figures/results_1a.pdf}}
\label{fig:graphe1a}
\hfill
\subfloat[Hit Rate]{\includegraphics[trim=3.4cm 9.5cm 4.3cm 9.91cm,width = 0.42\textwidth]{Figures/results_1b.pdf}}
\label{fig:graphe1b}
\caption{The impact of the signal-to-noise ratio on the performance metrics of the various methods is depicted. The solid and dashed lines correspond to the localization performance for the client and non-client targets, respectively.}
\label{fig:graphe1}
\end{figure*}
This section evaluates the enhancement brought by the exploitation of the BFFs at the PWR on the accuracy of the radar in localizing targets within its coverage area. The joint NDP and BFF processing outlined in Section \ref{sec:BBF_Radar_Process} is compared through $30,000$ simulations with two different methods:
\begin{enumerate}
\item \textbf{MUSIC NDP:} This method relies solely on information from the NDP and does not utilize the additional data from the BFF. In this approach, the target positions are determined directly from the pre-estimations $\widehat{\varphi}_{k}$ and $\widehat{\vartheta}_{k}$ obtained using the MUSIC algorithm.
\item \textbf{MUSIC NDP+BFF:} In this method, the MUSIC pseudo-spectra from both the NDP and the BFFs are combined onto a common $x-y$ map. A peak detection algorithm is then applied to determine the target positions.
\end{enumerate}
To compare these methods, the following performance metrics
are studied:
\begin{enumerate}
\item \textbf{Hit Rate:} A hit is acknowledged when a peak is detected within a vicinity of 2 meters from the true target position; otherwise, it is considered a miss.
\item \textbf{RMSE:} The root mean square error (RMSE) is computed between the true target position and the corresponding detected position. To ensure a fair comparison between the methods, only the targets resulting in a hit by all methods are considered in the evaluation of the RMSE.
\end{enumerate}

\balance For each simulation, we analyze a fixed AP and PWR setup designated to locate two client targets and a non-client target randomly positioned. The number of antennas are $N_A=N_u=N_P=4$ and the number of subcarriers is $Q=512$.
\figurename~\ref{fig:graphe1} depicts the results obtained for the hit rate and the RMSE for the client and non client targets as functions of the SNR. The SNR is defined here as the mean of the quotient of the radar channel coefficients of each path by the noise variance. Note that the same noise variance is considered at the clients and the PWR. It is observed that for both the client and the non-client target, the hybrid fusion of the NDP and the BFF based on the alternating summation method enhances the achievable RMSE compared to the exploitation of the NDP only.  Regarding the hit rate, the alternating summation presents similar performance at high SNRs as the NDP-based MUSIC. At low SNRs, we observe that it improves the hit rate for the client targets. However, it can decrease the hit rate of the non-client target since the association step is not always well performed at low SNRs. We can also observe that the method to combine the information from the NDP and from the BFF is important, as a simple combination of MUSIC pseudo-spectrums deteriorates the RMSE. Furthermore, it can be observed that the alternating projection method achieves an improved RMSE for the client target compared to the non-client one. This results from the improved ability of the alternating summation method to account for the varying localization ability of the NDP and the BFF. Globally, these results confirm the benefit of the hybrid combination when the fusion rule is appropriately chosen.
